Relative Pose Estimation through Affine Corrections of Monocular Depth Priors

Monocular depth estimation (MDE) models have undergone significant advancements over recent years. Many MDE models aim to predict affine-invariant relative depth from monocular images, while recent developments in large-scale training and vision foundation models enable reasonable estimation of metric (absolute) depth. However, effectively leveraging these predictions for geometric vision tasks, in particular relative pose estimation, remains relatively under explored. While depths provide rich constraints for cross-view image alignment, the intrinsic noise and ambiguity from the monocular depth priors present practical challenges to improving upon classic keypoint-based solutions. In this paper, we develop three solvers for relative pose estimation that explicitly account for independent affine (scale and shift) ambiguities, covering both calibrated and uncalibrated conditions. We further propose a hybrid estimation pipeline that combines our proposed solvers with classic point-based solvers and epipolar constraints. We find that the affine correction modeling is beneficial to not only the relative depth priors but also, surprisingly, the "metric" ones. Results across multiple datasets demonstrate large improvements of our approach over classic keypoint-based baselines and PnP-based solutions, under both calibrated and uncalibrated setups. We also show that our method improves consistently with different feature matchers and MDE models, and can further benefit from very recent advances on both modules. Code is available at https://github.com/MarkYu98/madpose.

==> figures/vis_scale_only.tex <==
\begin{figure}[tb]
\scriptsize
\centering
\setlength\tabcolsep{3pt} % default value: 6pt

\begin{minipage}{.95\linewidth}
\renewcommand{\arraystretch}{0.4}
\begin{tabular}{cccc}
\includegraphics[width=0.15\linewidth]{images/vis_samples/107_0.png} &
\raisebox{-0.5\height}[0pt][0pt]{\includegraphics[width=0.24\linewidth]{images/vis_samples/107-scaleonly.png}} &
\raisebox{-0.5\height}[0pt][0pt]{\includegraphics[width=0.24\linewidth]{images/vis_samples/107-ours.png}} &
\raisebox{-0.5\height}[0pt][0pt]{\includegraphics[width=0.24\linewidth]{images/vis_samples/107-gt.png}} \\
\includegraphics[width=0.15\linewidth]{images/vis_samples/107_1.png} 
\end{tabular}
\end{minipage} 
\caption{Visualization of aligned point clouds with (left to right): the scale-only ablated baseline, our method, and GT on an image pair from ScanNet-1500\cite{dai2017scannet}.
\RP{Where is this referenced in the text?}}
\label{fig:vis_samples_scale_only}
\end{figure}


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Recently, deep learning-based monocular depth estimation (MDE) has made remarkable progress~\cite{birkl2023midas3.1, kar20223d-omnidata, marigold, depthanything, depth_anything_v2, wang2024moge}, offering increasingly accurate 3D information from single 2D images. These advancements have opened up new possibilities for enriching traditional geometric computer vision tasks with 3D priors. The ability to infer depth information from a single image has been shown to have useful implications in applications like autonomous navigation\todo{add citations}~\cite{}, ...~\cite{}.

Despite the significant progress in monocular depth estimation, the integration of these depth priors into fundamental geometric computer vision tasks, particularly camera pose estimation, remains under-studied. While incorporating depth information would be beneficial intuitively, effectively leveraging these priors to find geometric relationships between multiple views presents unique challenges that have not been fully addressed by existing works~\cite{studiosfm, barath2022relative, ding2024fundamental}.

A critical limitation of existing approaches is the common assumption that predicted depth maps from different views can be related by a single scale factor. This assumption, however, fails to account for the intrinsic properties of modern monocular depth estimation models. State-of-the-art depth predictors~\cite{marigold, depth_anything_v2, wang2024moge} typically produce relative depth or disparity (inverse-depth) that are invariant to both scale and shift (affine) transformations.

In this paper, we propose three solvers specialized for solving relative pose problems in three different cases. These solvers use pixel correspondences along with their corresponding affine-invariant depth priors, and are able to explicitly model both scale and shift variations in the depth predictions. The solvers work on image pairs that are either:
\begin{itemize} \itemsep0pt
    \item captured by cameras with calibrated intrinsics.
    \item captured with cameras of a common unknown focal length (shared-focal).
    \item captured with two unknown focal length cameras.
\end{itemize}

In addition, we integrate these new solvers into a flexible hybrid RANSAC estimation pipeline, which combines our depth-aware solvers with classic point-based solvers~\cite{Nister03FivePt,hartley_zisserman_2004,Stewenius2008}, creating a robust framework that jointly optimizes both the classical epipolar constraints and the reprojections of points using depth, leveraging the strengths of both approaches. By doing so, we achieved improved accuracy and robustness of relative pose estimation across different datasets.

The key contributions of our work can be summarized as follows:
\begin{itemize}
    \item We introduce a novel formulation for solving relative pose with explicitly modeling of the scale-and-shift invariance inherent in modern monocular depth predictions, addressing a limitation in existing methods.
    \item We develop three new solvers tailored to different camera setups, providing a comprehensive solution for various practical scenarios.
    \item Our hybrid estimation pipeline integrates depth-aware and classic point-based solvers, resulting in improved accuracy and robustness in relative pose estimation tasks.
    \item Our framework is compatible with a wide range of correspondence matching techniques and monocular depth estimation models, which is easily applicable and extendable.
\end{itemize}

